"The Squawk Bot": Joint Learning of Time Series and Text Data Modalities for Automated Financial Information Filtering

Multimodal analysis that uses numerical time series and textual corpora as input data sources is becoming a promising approach, especially in the financial industry. However, the main focus of such analysis has been on achieving high prediction accuracy while little effort has been spent on the important task of understanding the association between the two data modalities. Performance on the time series hence receives little explanation though human-understandable textual information is available. In this work, we address the problem of given a numerical time series, and a general corpus of textual stories collected in the same period of the time series, the task is to timely discover a succinct set of textual stories associated with that time series. Towards this goal, we propose a novel multi-modal neural model called MSIN that jointly learns both numerical time series and categorical text articles in order to unearth the association between them. Through multiple steps of data interrelation between the two data modalities, MSIN learns to focus on a small subset of text articles that best align with the performance in the time series. This succinct set is timely discovered and presented as recommended documents, acting as automated information filtering, for the given time series. We empirically evaluate the performance of our model on discovering relevant news articles for two stock time series from Apple and Google companies, along with the daily news articles collected from the Thomson Reuters over a period of seven consecutive years. The experimental results demonstrate that MSIN achieves up to 84.9% and 87.2% in recalling the ground truth articles respectively to the two examined time series, far more superior to state-of-the-art algorithms that rely on conventional attention mechanism in deep learning.

==> AAPL-ATTN-SMALL.tex <==
\begin{table}%[htbp]
\centering
  \caption{AAPL: News headlines from 3 days in 2013 (test set). Succinct set of relevant news in MSIN is blue-highlighted by setting: accumulated probability mass $\geq 50\%$. (ref. to Appendix~\ref{AG-ATTN-ALL})}
  \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}[t]{llll}
    \toprule
    GRUtxt & LSTMw/o & MSIN & News headlines \\
    \midrule
          &       &       & Date: 2013-01-22 \\
    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!15}{\makebox[3em]{\strut {0.15}}}  &  \colorbox{green!0}{\strut 02.  japan government welcome boj ease step towards percent inflation } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!21}{\makebox[3em]{\strut {0.21}}}  &  \colorbox{green!21}{\strut 04.  instant view existing home sale fall december } \\
    \colorbox{violet!14}{\makebox[3em]{\strut {0.14}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!8}{\makebox[3em]{\strut {0.09}}}  &  \colorbox{green!0}{\strut 05.  german exporter fear devaluation round boj move } \\
    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 07.  home resale fall housing recovery still track } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!13}{\makebox[3em]{\strut {0.14}}}  & \colorbox{green!39}{\makebox[3em]{\strut {0.40}}}  &  \colorbox{green!39}{\strut 13.  steve jobs threaten patent suit no hire policy filing } \\
    \midrule
          &       &       & Date: 2013-08-14 \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 06.  j.c. penney share spike report sale improve august } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  analysis balloon google experiment web access } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 09.  wallstreet fall uncertainty fed bond buying } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!75}{\makebox[3em]{\strut {0.76}}}  &  \colorbox{green!75}{\strut 10.  apple face possible may trial e book damage } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!17}{\makebox[3em]{\strut {0.17}}}  &  \colorbox{green!0}{\strut 11.  japan government spokesman no pm abe corporate tax cut } \\
    \midrule
          &       &       & Date: 2013-09-06 \\
    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!20}{\makebox[3em]{\strut {0.21}}}  &  \colorbox{green!20}{\strut 01.  china unicom telecom sell late iphone shortly us launch } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!5}{\makebox[3em]{\strut {0.05}}}  &  \colorbox{green!0}{\strut 06.  wind down market street funding amid regulatory pressure } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!9}{\makebox[3em]{\strut {0.09}}}  &  \colorbox{green!0}{\strut 11.  g20 say economy recover but no end crisis yet } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!37}{\makebox[3em]{\strut {0.37}}}  &  \colorbox{green!37}{\strut 16.  apple hit us injunction e books antitrust case } \\
    \colorbox{violet!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 23.  cost lack indonesia economy } \\
    \bottomrule
    \end{tabular}%
  }
  \label{tab:AAPL-attn}%
\end{table}

==> AAPL-GOOG-news.tex <==
\begin{table}%[htbp]
\captionsetup{font=scriptsize}
\parbox[t]{.49\linewidth}{
\centering
  \caption{AAPL dataset: News headlines from 3 days in 2013 (test set). Succinct set of relevant news in AsyncLSTM is blue-highlighted by setting: accumulated probability mass $\geq 50\%$.}
  \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}[t]{llll}
    \toprule
    GRUtxt & LSTMw/o & AsyncLSTM & News headlines \\
    \midrule
          &       &       & Date: 2013-01-22 \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!21}{\makebox[3em]{\strut {0.21}}}  &  \colorbox{green!21}{\strut 04.  instant view existing home sale fall december } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!13}{\makebox[3em]{\strut {0.14}}}  & \colorbox{green!39}{\makebox[3em]{\strut {0.40}}}  &  \colorbox{green!39}{\strut 13.  steve jobs threaten patent suit no hire policy filing } \\
    \midrule
          &       &       & Date: 2013-08-14 \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!75}{\makebox[3em]{\strut {0.76}}}  &  \colorbox{green!75}{\strut 10.  apple face possible may trial e book damage } \\
    \midrule
          &       &       & Date: 2013-09-06 \\
    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!20}{\makebox[3em]{\strut {0.21}}}  &  \colorbox{green!20}{\strut 01.  china unicom telecom sell late iphone shortly us launch } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!37}{\makebox[3em]{\strut {0.37}}}  &  \colorbox{green!37}{\strut 16.  apple hit us injunction e books antitrust case } \\
    \bottomrule
    \end{tabular}%
  }
  \label{tab:AAPL-attn}%
}
\hfill
\parbox[t]{.5\linewidth}{
 \centering
  \caption{GOOG dataset: News headlines from 3 days in 2013 (test set). Succinct set of relevant news in AsyncLSTM is blue-highlighted by setting: accumulated probability mass $\geq 50\%$.}
  \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}[t]{llll}
    \toprule
    GRUtxt & LSTMw/o & AsyncLSTM & News headlines \\
    \midrule
          &       &       & Date: 2013-01-09 \\
    \colorbox{violet!26}{\makebox[3em]{\strut {0.26}}}  & \colorbox{orange!52}{\makebox[3em]{\strut {0.52}}}  & \colorbox{green!87}{\makebox[3em]{\strut {0.87}}}  &  \colorbox{green!87}{\strut 02.  google drop key patent claim microsoft } \\
    \midrule
          &       &       & Date: 2013-08-14 \\
    \colorbox{violet!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!17}{\makebox[3em]{\strut {0.18}}}  & \colorbox{green!79}{\makebox[3em]{\strut {0.79}}}  &  \colorbox{green!79}{\strut 08.  analysis balloon google experiment web access } \\
    \midrule
          &       &       & Date: 2013-08-29 \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!20}{\makebox[3em]{\strut {0.20}}}  &  \colorbox{green!20}{\strut 04.  china environment min suspends approval cnpc } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!37}{\makebox[3em]{\strut {0.37}}}  &  \colorbox{green!37}{\strut 16.  china google power global drive } \\
    \bottomrule
    \end{tabular}%
  }
  \label{tab:GOOG-attn}%
}
\end{table}



%\begin{table}[htbp]
%  \centering
%  \caption{AAPL dataset: News headlines from 3 days in 2013 (test set). Succinct set of relevant news in AsyncLSTM is blue-highlighted by setting: accumulated probability mass $\geq 50\%$.}
%  \resizebox{0.45\textwidth}{!}{%
%    \begin{tabular}{llll}
%    \toprule
%    GRUtxt & LSTMw/o & AsyncLSTM & News headlines \\
%    \midrule
%          &       &       & 1/22/13 \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!0}{\makebox[3em]{\strut {0.00}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  analysis no respite euro zone long rebalancing slog } \\
%    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!15}{\makebox[3em]{\strut {0.15}}}  &  \colorbox{green!0}{\strut 02.  japan government welcome boj ease step towards percent inflation } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 03.  japan government panel need achieve budget surplus } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!21}{\makebox[3em]{\strut {0.21}}}  &  \colorbox{green!21}{\strut 04.  instant view existing home sale fall december } \\
%    \colorbox{violet!14}{\makebox[3em]{\strut {0.14}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!8}{\makebox[3em]{\strut {0.09}}}  &  \colorbox{green!0}{\strut 05.  german exporter fear devaluation round boj move } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 06.  bank japan yet revive economy } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 07.  home resale fall housing recovery still track } \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  instant view google put up well than expect quarterly number } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 09.  bank japan buy asset sp set new five year high } \\
%    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 10.  google fourth quarter result shine ad rate decline slows } \\
%    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 11.  banks commodity stock lift sp five year high } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 12.  google fourth quarter result shine ad rate decline slows } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!13}{\makebox[3em]{\strut {0.14}}}  & \colorbox{green!39}{\makebox[3em]{\strut {0.40}}}  &  \colorbox{green!39}{\strut 13.  steve jobs threaten patent suit no hire policy filing } \\
%    \midrule
%          &       &       & 8/14/13 \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  france exit recession beat second quarter gdp forecast } \\
%    \colorbox{violet!9}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!14}{\makebox[3em]{\strut {0.14}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 02.  euro zone performance suggests recovery sight european rehn } \\
%    \colorbox{violet!14}{\makebox[3em]{\strut {0.14}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  germany france haul euro zone recession } \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  yellen see likely next fed chair despite summers chatter reuters poll } \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 05.  us modest recovery fed cut back qe next month reuters poll } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 06.  j.c. penney share spike report sale improve august } \\
%    \colorbox{violet!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 07.  wallstreet end down fed uncertainty data boost europe } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  analysis balloon google experiment web access } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 09.  wallstreet fall uncertainty fed bond buying } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!75}{\makebox[3em]{\strut {0.76}}}  &  \colorbox{green!75}{\strut 10.  apple face possible may trial e book damage } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!17}{\makebox[3em]{\strut {0.17}}}  &  \colorbox{green!0}{\strut 11.  japan government spokesman no pm abe corporate tax cut } \\
%    \midrule
%          &       &       & 9/6/13 \\
%    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!20}{\makebox[3em]{\strut {0.21}}}  &  \colorbox{green!20}{\strut 01.  china unicom telecom sell late iphone shortly us launch } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 02.  spain industrial output fall month july } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  french consumer confidence trade point improve outlook } \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  uk industrial output flat july trade deficit widens sharply } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 05.  boj kuroda room policy response tax hike hurt economy minute } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!5}{\makebox[3em]{\strut {0.05}}}  &  \colorbox{green!0}{\strut 06.  wind down market street funding amid regulatory pressure } \\
%    \colorbox{violet!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 07.  china able cope fed policy taper central bank head } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  instant view us august nonfarm payroll rise } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 09.  analysis fed shift syria crisis trading strategy } \\
%    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 10.  factbox three thing learn us job report } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!9}{\makebox[3em]{\strut {0.09}}}  &  \colorbox{green!0}{\strut 11.  g20 say economy recover but no end crisis yet } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 12.  us regulator talk european energy price probe } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 13.  wallstreet flat job data syria worry spur caution } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 14.  job growth disappoints offer note fed } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 15.  bond yield dollar fall us job data } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!37}{\makebox[3em]{\strut {0.37}}}  &  \colorbox{green!37}{\strut 16.  apple hit us injunction e books antitrust case } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 17.  wallstreet week ahead markets could turn choppy fed syria risk mount } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 18.  china buy giant kazakh oilfield billion } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!1}{\strut 19.  italy wo n't block foreign takeover economy minister } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 20.  china august export beat forecast point stabilization } \\
%    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!06}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 21.  wallstreet week ahead markets could turn choppy fed syria risk mount } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 22.  india inc policymakers shape up ship } \\
%    \colorbox{violet!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 23.  cost lack indonesia economy } \\
%    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 24.  mexico proposes new tax regime pemex } \\
%    \bottomrule
%    \end{tabular}%
%  }
%  \label{tab:addlabel}%
%\end{table}%
%





%\begin{table}[htbp]
%  \centering
%  \caption{GOOG dataset: News headlines from 3 days in 2013 (test set). Succinct set of relevant news in AsyncLSTM is blue-highlighted by setting: accumulated probability mass $\geq 50\%$.}
%  \resizebox{0.45\textwidth}{!}{%
%    \begin{tabular}{llll}
%    \toprule
%    GRUtxt & LSTMw/o & AsyncLSTM & News headlines \\
%    \midrule
%          &       &       & 1/9/13 \\
%    \colorbox{violet!23}{\makebox[3em]{\strut {0.23}}}  & \colorbox{orange!34}{\makebox[3em]{\strut {0.34}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  short sellers circle stock confidence waver } \\
%    \colorbox{violet!26}{\makebox[3em]{\strut {0.26}}}  & \colorbox{orange!52}{\makebox[3em]{\strut {0.52}}}  & \colorbox{green!87}{\makebox[3em]{\strut {0.87}}}  &  \colorbox{green!87}{\strut 02.  google drop key patent claim microsoft } \\
%    \colorbox{violet!21}{\makebox[3em]{\strut {0.21}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  alcoa result lift share dollar up vs. yen } \\
%    \colorbox{violet!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  wallstreet rise alcoa report earnings } \\
%    \midrule
%          &       &       & 8/14/13 \\
%    \colorbox{violet!10}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  france exit recession beat second quarter gdp forecast } \\
%    \colorbox{violet!9}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 02.  euro zone performance suggests recovery sight european rehn } \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  germany france haul euro zone recession } \\
%    \colorbox{violet!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  yellen see likely next fed chair despite summers chatter reuters poll } \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 05.  us modest recovery fed cut back qe next month reuters poll } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 06.  j.c. penney share spike report sale improve august } \\
%    \colorbox{violet!9}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 07.  wallstreet end down fed uncertainty data boost europe } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!17}{\makebox[3em]{\strut {0.18}}}  & \colorbox{green!79}{\makebox[3em]{\strut {0.79}}}  &  \colorbox{green!79}{\strut 08.  analysis balloon google experiment web access } \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.09}}}  & \colorbox{orange!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 09.  wallstreet fall uncertainty fed bond buying } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!16}{\makebox[3em]{\strut {0.16}}}  & \colorbox{green!5}{\makebox[3em]{\strut {0.05}}}  &  \colorbox{green!0}{\strut 10.  apple face possible may trial e book damage } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 11.  japan government spokesman no pm abe corporate tax cut } \\
%    \midrule
%          &       &       & 8/29/13 \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 01.  india pm likely make statement economy friday } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 02.  boj warns emerge market may see outflow } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 03.  european rehn say lender step up assessment greece next month } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!20}{\makebox[3em]{\strut {0.20}}}  &  \colorbox{green!20}{\strut 04.  china environment min suspends approval cnpc } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!7}{\makebox[3em]{\strut {0.08}}}  &  \colorbox{green!0}{\strut 05.  italy still meet target scrap property tax say rehn } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!1}{\strut 06.  spain economic slump longer than thought but ease } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 07.  india central bank consider gold trade minister } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  rupee fall front slow indian economy } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 09.  india rupee bounce record low pm may address economy } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 10.  exclusive india might buy gold ease rupee crisis } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 11.  spain recession longer than thought but close end } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 12.  india finance minister asks bank ensure credit flow industry } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 13.  easing stimulus weigh oil next year reuters poll } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 14.  exclusive india might buy gold ease rupee crisis } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 15.  india rupee bounce record low government seek solution } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!37}{\makebox[3em]{\strut {0.37}}}  &  \colorbox{green!37}{\strut 16.  china google power global drive } \\
%    \colorbox{violet!09}{\makebox[3em]{\strut {0.09}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 17.  gdp growth beat forecast may boost case fed move } \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.01}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 18.  wallstreet rise economy but syria concern limit gain } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.01}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 19.  oil dip syria action uncertain dollar rise data } \\
%    \colorbox{violet!1}{\makebox[3em]{\strut {0.02}}}  & \colorbox{orange!0}{\makebox[3em]{\strut {0.00}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 20.  boe carney say uncertainty rbs future end } \\
%    \end{tabular}%
%  }
%  \label{tab:addlabel}%
%\end{table}%
%




==> AAPL-GOOG-news5.tex <==
%\vspace*{-0.3cm}
\begin{table}%[htbp]
\captionsetup{font=scriptsize}
\parbox[t]{.49\linewidth}{
\centering
  \caption{AAPL: News headlines from 3 days in 2013 (test set). Succinct set of relevant news in AsyncLSTM is blue-highlighted by setting: accumulated probability mass $\geq 50\%$. (ref. to Appendix~\ref{AG-ATTN-ALL})}
  \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}[t]{llll}
    \toprule
    GRUtxt & LSTMw/o & AsyncLSTM & News headlines \\
    \midrule
          &       &       & Date: 2013-01-22 \\
    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!15}{\makebox[3em]{\strut {0.15}}}  &  \colorbox{green!0}{\strut 02.  japan government welcome boj ease step towards percent inflation } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!21}{\makebox[3em]{\strut {0.21}}}  &  \colorbox{green!21}{\strut 04.  instant view existing home sale fall december } \\
    \colorbox{violet!14}{\makebox[3em]{\strut {0.14}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!8}{\makebox[3em]{\strut {0.09}}}  &  \colorbox{green!0}{\strut 05.  german exporter fear devaluation round boj move } \\
    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 07.  home resale fall housing recovery still track } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!13}{\makebox[3em]{\strut {0.14}}}  & \colorbox{green!39}{\makebox[3em]{\strut {0.40}}}  &  \colorbox{green!39}{\strut 13.  steve jobs threaten patent suit no hire policy filing } \\
    \midrule
          &       &       & Date: 2013-08-14 \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 06.  j.c. penney share spike report sale improve august } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  analysis balloon google experiment web access } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 09.  wallstreet fall uncertainty fed bond buying } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!75}{\makebox[3em]{\strut {0.76}}}  &  \colorbox{green!75}{\strut 10.  apple face possible may trial e book damage } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!17}{\makebox[3em]{\strut {0.17}}}  &  \colorbox{green!0}{\strut 11.  japan government spokesman no pm abe corporate tax cut } \\
    \midrule
          &       &       & Date: 2013-09-06 \\
    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!20}{\makebox[3em]{\strut {0.21}}}  &  \colorbox{green!20}{\strut 01.  china unicom telecom sell late iphone shortly us launch } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!5}{\makebox[3em]{\strut {0.05}}}  &  \colorbox{green!0}{\strut 06.  wind down market street funding amid regulatory pressure } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!9}{\makebox[3em]{\strut {0.09}}}  &  \colorbox{green!0}{\strut 11.  g20 say economy recover but no end crisis yet } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!37}{\makebox[3em]{\strut {0.37}}}  &  \colorbox{green!37}{\strut 16.  apple hit us injunction e books antitrust case } \\
    \colorbox{violet!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 23.  cost lack indonesia economy } \\
    \bottomrule
    \end{tabular}%
  }
  \label{tab:AAPL-attn}%
}
\hfill
\parbox[t]{.5\linewidth}{
 \centering
  \caption{GOOG: News headlines from 3 days in 2013 (test set). Succinct set of relevant news in AsyncLSTM is blue-highlighted by setting: accumulated probability mass $\geq 50\%$.(ref. to Appendix~\ref{AG-ATTN-ALL})}
  \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}[t]{llll}
    \toprule
    GRUtxt & LSTMw/o & AsyncLSTM & News headlines \\
    \midrule
          &       &       & Date: 2013-01-09 \\
    \colorbox{violet!23}{\makebox[3em]{\strut {0.23}}}  & \colorbox{orange!34}{\makebox[3em]{\strut {0.34}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  short sellers circle stock confidence waver } \\
    \colorbox{violet!26}{\makebox[3em]{\strut {0.26}}}  & \colorbox{orange!52}{\makebox[3em]{\strut {0.52}}}  & \colorbox{green!87}{\makebox[3em]{\strut {0.87}}}  &  \colorbox{green!87}{\strut 02.  google drop key patent claim microsoft } \\
    \colorbox{violet!21}{\makebox[3em]{\strut {0.21}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  alcoa result lift share dollar up vs. yen } \\
    \colorbox{violet!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  wallstreet rise alcoa report earnings } \\
    \midrule
          &       &       & Date: 2013-08-14 \\
    \colorbox{violet!10}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  france exit recession beat second quarter gdp forecast } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 06.  j.c. penney share spike report sale improve august } \\
    \colorbox{violet!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!17}{\makebox[3em]{\strut {0.18}}}  & \colorbox{green!79}{\makebox[3em]{\strut {0.79}}}  &  \colorbox{green!79}{\strut 08.  analysis balloon google experiment web access } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!16}{\makebox[3em]{\strut {0.16}}}  & \colorbox{green!5}{\makebox[3em]{\strut {0.05}}}  &  \colorbox{green!0}{\strut 10.  apple face possible may trial e book damage } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 11.  japan government spokesman no pm abe corporate tax cut } \\
    \midrule
          &       &       & Date: 2013-08-29 \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 03.  european rehn say lender step up assessment greece next month } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!20}{\makebox[3em]{\strut {0.20}}}  &  \colorbox{green!20}{\strut 04.  china environment min suspends approval cnpc } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!7}{\makebox[3em]{\strut {0.08}}}  &  \colorbox{green!0}{\strut 05.  italy still meet target scrap property tax say rehn } \\    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!37}{\makebox[3em]{\strut {0.37}}}  &  \colorbox{green!37}{\strut 16.  china google power global drive } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.01}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 19.  oil dip syria action uncertain dollar rise data } \\
    \bottomrule
    \end{tabular}%
  }
  \label{tab:GOOG-attn}%
}
\vspace*{-0.63cm}
\end{table}




%\begin{table}[htbp]
%  \centering
%  \caption{AAPL dataset: News headlines from 3 days in 2013 (test set). Succinct set of relevant news in AsyncLSTM is blue-highlighted by setting: accumulated probability mass $\geq 50\%$.}
%  \resizebox{0.45\textwidth}{!}{%
%    \begin{tabular}{llll}
%    \toprule
%    GRUtxt & LSTMw/o & AsyncLSTM & News headlines \\
%    \midrule
%          &       &       & 1/22/13 \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!0}{\makebox[3em]{\strut {0.00}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  analysis no respite euro zone long rebalancing slog } \\
%    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!15}{\makebox[3em]{\strut {0.15}}}  &  \colorbox{green!0}{\strut 02.  japan government welcome boj ease step towards percent inflation } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 03.  japan government panel need achieve budget surplus } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!21}{\makebox[3em]{\strut {0.21}}}  &  \colorbox{green!21}{\strut 04.  instant view existing home sale fall december } \\
%    \colorbox{violet!14}{\makebox[3em]{\strut {0.14}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!8}{\makebox[3em]{\strut {0.09}}}  &  \colorbox{green!0}{\strut 05.  german exporter fear devaluation round boj move } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 06.  bank japan yet revive economy } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 07.  home resale fall housing recovery still track } \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  instant view google put up well than expect quarterly number } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 09.  bank japan buy asset sp set new five year high } \\
%    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 10.  google fourth quarter result shine ad rate decline slows } \\
%    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 11.  banks commodity stock lift sp five year high } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 12.  google fourth quarter result shine ad rate decline slows } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!13}{\makebox[3em]{\strut {0.14}}}  & \colorbox{green!39}{\makebox[3em]{\strut {0.40}}}  &  \colorbox{green!39}{\strut 13.  steve jobs threaten patent suit no hire policy filing } \\
%    \midrule
%          &       &       & 8/14/13 \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  france exit recession beat second quarter gdp forecast } \\
%    \colorbox{violet!9}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!14}{\makebox[3em]{\strut {0.14}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 02.  euro zone performance suggests recovery sight european rehn } \\
%    \colorbox{violet!14}{\makebox[3em]{\strut {0.14}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  germany france haul euro zone recession } \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  yellen see likely next fed chair despite summers chatter reuters poll } \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 05.  us modest recovery fed cut back qe next month reuters poll } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 06.  j.c. penney share spike report sale improve august } \\
%    \colorbox{violet!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 07.  wallstreet end down fed uncertainty data boost europe } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  analysis balloon google experiment web access } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 09.  wallstreet fall uncertainty fed bond buying } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!75}{\makebox[3em]{\strut {0.76}}}  &  \colorbox{green!75}{\strut 10.  apple face possible may trial e book damage } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!17}{\makebox[3em]{\strut {0.17}}}  &  \colorbox{green!0}{\strut 11.  japan government spokesman no pm abe corporate tax cut } \\
%    \midrule
%          &       &       & 9/6/13 \\
%    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!20}{\makebox[3em]{\strut {0.21}}}  &  \colorbox{green!20}{\strut 01.  china unicom telecom sell late iphone shortly us launch } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 02.  spain industrial output fall month july } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  french consumer confidence trade point improve outlook } \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  uk industrial output flat july trade deficit widens sharply } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 05.  boj kuroda room policy response tax hike hurt economy minute } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!5}{\makebox[3em]{\strut {0.05}}}  &  \colorbox{green!0}{\strut 06.  wind down market street funding amid regulatory pressure } \\
%    \colorbox{violet!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 07.  china able cope fed policy taper central bank head } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  instant view us august nonfarm payroll rise } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 09.  analysis fed shift syria crisis trading strategy } \\
%    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 10.  factbox three thing learn us job report } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!9}{\makebox[3em]{\strut {0.09}}}  &  \colorbox{green!0}{\strut 11.  g20 say economy recover but no end crisis yet } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 12.  us regulator talk european energy price probe } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 13.  wallstreet flat job data syria worry spur caution } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 14.  job growth disappoints offer note fed } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 15.  bond yield dollar fall us job data } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!37}{\makebox[3em]{\strut {0.37}}}  &  \colorbox{green!37}{\strut 16.  apple hit us injunction e books antitrust case } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 17.  wallstreet week ahead markets could turn choppy fed syria risk mount } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 18.  china buy giant kazakh oilfield billion } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!1}{\strut 19.  italy wo n't block foreign takeover economy minister } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 20.  china august export beat forecast point stabilization } \\
%    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!06}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 21.  wallstreet week ahead markets could turn choppy fed syria risk mount } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 22.  india inc policymakers shape up ship } \\
%    \colorbox{violet!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 23.  cost lack indonesia economy } \\
%    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 24.  mexico proposes new tax regime pemex } \\
%    \bottomrule
%    \end{tabular}%
%  }
%  \label{tab:addlabel}%
%\end{table}%
%





%\begin{table}[htbp]
%  \centering
%  \caption{GOOG dataset: News headlines from 3 days in 2013 (test set). Succinct set of relevant news in AsyncLSTM is blue-highlighted by setting: accumulated probability mass $\geq 50\%$.}
%  \resizebox{0.45\textwidth}{!}{%
%    \begin{tabular}{llll}
%    \toprule
%    GRUtxt & LSTMw/o & AsyncLSTM & News headlines \\
%    \midrule
%          &       &       & 1/9/13 \\
%    \colorbox{violet!23}{\makebox[3em]{\strut {0.23}}}  & \colorbox{orange!34}{\makebox[3em]{\strut {0.34}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  short sellers circle stock confidence waver } \\
%    \colorbox{violet!26}{\makebox[3em]{\strut {0.26}}}  & \colorbox{orange!52}{\makebox[3em]{\strut {0.52}}}  & \colorbox{green!87}{\makebox[3em]{\strut {0.87}}}  &  \colorbox{green!87}{\strut 02.  google drop key patent claim microsoft } \\
%    \colorbox{violet!21}{\makebox[3em]{\strut {0.21}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  alcoa result lift share dollar up vs. yen } \\
%    \colorbox{violet!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  wallstreet rise alcoa report earnings } \\
%    \midrule
%          &       &       & 8/14/13 \\
%    \colorbox{violet!10}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  france exit recession beat second quarter gdp forecast } \\
%    \colorbox{violet!9}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 02.  euro zone performance suggests recovery sight european rehn } \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  germany france haul euro zone recession } \\
%    \colorbox{violet!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  yellen see likely next fed chair despite summers chatter reuters poll } \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 05.  us modest recovery fed cut back qe next month reuters poll } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 06.  j.c. penney share spike report sale improve august } \\
%    \colorbox{violet!9}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 07.  wallstreet end down fed uncertainty data boost europe } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!17}{\makebox[3em]{\strut {0.18}}}  & \colorbox{green!79}{\makebox[3em]{\strut {0.79}}}  &  \colorbox{green!79}{\strut 08.  analysis balloon google experiment web access } \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.09}}}  & \colorbox{orange!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 09.  wallstreet fall uncertainty fed bond buying } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!16}{\makebox[3em]{\strut {0.16}}}  & \colorbox{green!5}{\makebox[3em]{\strut {0.05}}}  &  \colorbox{green!0}{\strut 10.  apple face possible may trial e book damage } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 11.  japan government spokesman no pm abe corporate tax cut } \\
%    \midrule
%          &       &       & 8/29/13 \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 01.  india pm likely make statement economy friday } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 02.  boj warns emerge market may see outflow } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 03.  european rehn say lender step up assessment greece next month } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!20}{\makebox[3em]{\strut {0.20}}}  &  \colorbox{green!20}{\strut 04.  china environment min suspends approval cnpc } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!7}{\makebox[3em]{\strut {0.08}}}  &  \colorbox{green!0}{\strut 05.  italy still meet target scrap property tax say rehn } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!1}{\strut 06.  spain economic slump longer than thought but ease } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 07.  india central bank consider gold trade minister } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  rupee fall front slow indian economy } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 09.  india rupee bounce record low pm may address economy } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 10.  exclusive india might buy gold ease rupee crisis } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 11.  spain recession longer than thought but close end } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 12.  india finance minister asks bank ensure credit flow industry } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 13.  easing stimulus weigh oil next year reuters poll } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 14.  exclusive india might buy gold ease rupee crisis } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 15.  india rupee bounce record low government seek solution } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!37}{\makebox[3em]{\strut {0.37}}}  &  \colorbox{green!37}{\strut 16.  china google power global drive } \\
%    \colorbox{violet!09}{\makebox[3em]{\strut {0.09}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 17.  gdp growth beat forecast may boost case fed move } \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.01}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 18.  wallstreet rise economy but syria concern limit gain } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.01}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 19.  oil dip syria action uncertain dollar rise data } \\
%    \colorbox{violet!1}{\makebox[3em]{\strut {0.02}}}  & \colorbox{orange!0}{\makebox[3em]{\strut {0.00}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 20.  boe carney say uncertainty rbs future end } \\
%    \end{tabular}%
%  }
%  \label{tab:addlabel}%
%\end{table}%
%




==> AAPL-GOOG-newsApendix.tex <==
%\begin{table}%[htbp]
\begin{table}[H]
\captionsetup{font=scriptsize}
\parbox[t]{.49\linewidth}{
\centering
  \caption{AAPL dataset: News headlines from 3 days in 2013 (test set). Succinct set of relevant news in AsyncLSTM is blue-highlighted by setting: accumulated probability mass $\geq 50\%$.}
  \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}[t]{llll}
    \toprule
    GRUtxt & LSTMw/o & AsyncLSTM & News headlines \\
    \midrule
          &       &       & Date: 2013-01-22 \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!0}{\makebox[3em]{\strut {0.00}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  analysis no respite euro zone long rebalancing slog } \\
    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!15}{\makebox[3em]{\strut {0.15}}}  &  \colorbox{green!0}{\strut 02.  japan government welcome boj ease step towards percent inflation } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 03.  japan government panel need achieve budget surplus } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!21}{\makebox[3em]{\strut {0.21}}}  &  \colorbox{green!21}{\strut 04.  instant view existing home sale fall december } \\
    \colorbox{violet!14}{\makebox[3em]{\strut {0.14}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!8}{\makebox[3em]{\strut {0.09}}}  &  \colorbox{green!0}{\strut 05.  german exporter fear devaluation round boj move } \\
    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 06.  bank japan yet revive economy } \\
    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 07.  home resale fall housing recovery still track } \\
    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  instant view google put up well than expect quarterly number } \\
    \colorbox{violet!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 09.  bank japan buy asset sp set new five year high } \\
    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 10.  google fourth quarter result shine ad rate decline slows } \\
    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 11.  banks commodity stock lift sp five year high } \\
    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 12.  google fourth quarter result shine ad rate decline slows } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!13}{\makebox[3em]{\strut {0.14}}}  & \colorbox{green!39}{\makebox[3em]{\strut {0.40}}}  &  \colorbox{green!39}{\strut 13.  steve jobs threaten patent suit no hire policy filing } \\
    \midrule
          &       &       & Date: 2013-08-14 \\
    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  france exit recession beat second quarter gdp forecast } \\
    \colorbox{violet!9}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!14}{\makebox[3em]{\strut {0.14}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 02.  euro zone performance suggests recovery sight european rehn } \\
    \colorbox{violet!14}{\makebox[3em]{\strut {0.14}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  germany france haul euro zone recession } \\
    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  yellen see likely next fed chair despite summers chatter reuters poll } \\
    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 05.  us modest recovery fed cut back qe next month reuters poll } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 06.  j.c. penney share spike report sale improve august } \\
    \colorbox{violet!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 07.  wallstreet end down fed uncertainty data boost europe } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  analysis balloon google experiment web access } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 09.  wallstreet fall uncertainty fed bond buying } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!75}{\makebox[3em]{\strut {0.76}}}  &  \colorbox{green!75}{\strut 10.  apple face possible may trial e book damage } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!17}{\makebox[3em]{\strut {0.17}}}  &  \colorbox{green!0}{\strut 11.  japan government spokesman no pm abe corporate tax cut } \\
    \midrule
          &       &       & Date: 2013-09-06 \\
    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!20}{\makebox[3em]{\strut {0.21}}}  &  \colorbox{green!20}{\strut 01.  china unicom telecom sell late iphone shortly us launch } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 02.  spain industrial output fall month july } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  french consumer confidence trade point improve outlook } \\
    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  uk industrial output flat july trade deficit widens sharply } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 05.  boj kuroda room policy response tax hike hurt economy minute } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!5}{\makebox[3em]{\strut {0.05}}}  &  \colorbox{green!0}{\strut 06.  wind down market street funding amid regulatory pressure } \\
    \colorbox{violet!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 07.  china able cope fed policy taper central bank head } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  instant view us august nonfarm payroll rise } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 09.  analysis fed shift syria crisis trading strategy } \\
    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 10.  factbox three thing learn us job report } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!9}{\makebox[3em]{\strut {0.09}}}  &  \colorbox{green!0}{\strut 11.  g20 say economy recover but no end crisis yet } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 12.  us regulator talk european energy price probe } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 13.  wallstreet flat job data syria worry spur caution } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 14.  job growth disappoints offer note fed } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 15.  bond yield dollar fall us job data } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!37}{\makebox[3em]{\strut {0.37}}}  &  \colorbox{green!37}{\strut 16.  apple hit us injunction e books antitrust case } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 17.  wallstreet week ahead markets could turn choppy fed syria risk mount } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 18.  china buy giant kazakh oilfield billion } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!1}{\strut 19.  italy wo n't block foreign takeover economy minister } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 20.  china august export beat forecast point stabilization } \\
    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!06}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 21.  wallstreet week ahead markets could turn choppy fed syria risk mount } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 22.  india inc policymakers shape up ship } \\
    \colorbox{violet!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 23.  cost lack indonesia economy } \\
    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 24.  mexico proposes new tax regime pemex } \\
    \bottomrule
    \end{tabular}%
  }
  \label{tab:AAPL-attn-Apnx}%
}
\hfill
\parbox[t]{.5\linewidth}{
 \centering
  \caption{GOOG dataset: News headlines from 3 days in 2013 (test set). Succinct set of relevant news in AsyncLSTM is blue-highlighted by setting: accumulated probability mass $\geq 50\%$.}
  \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}[t]{llll}
    \toprule
    GRUtxt & LSTMw/o & AsyncLSTM & News headlines \\
    \midrule
          &       &       & Date: 2013-01-09 \\
    \colorbox{violet!23}{\makebox[3em]{\strut {0.23}}}  & \colorbox{orange!34}{\makebox[3em]{\strut {0.34}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  short sellers circle stock confidence waver } \\
    \colorbox{violet!26}{\makebox[3em]{\strut {0.26}}}  & \colorbox{orange!52}{\makebox[3em]{\strut {0.52}}}  & \colorbox{green!87}{\makebox[3em]{\strut {0.87}}}  &  \colorbox{green!87}{\strut 02.  google drop key patent claim microsoft } \\
    \colorbox{violet!21}{\makebox[3em]{\strut {0.21}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  alcoa result lift share dollar up vs. yen } \\
    \colorbox{violet!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  wallstreet rise alcoa report earnings } \\
    \midrule
          &       &       & Date: 2013-08-14 \\
    \colorbox{violet!10}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  france exit recession beat second quarter gdp forecast } \\
    \colorbox{violet!9}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 02.  euro zone performance suggests recovery sight european rehn } \\
    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  germany france haul euro zone recession } \\
    \colorbox{violet!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  yellen see likely next fed chair despite summers chatter reuters poll } \\
    \colorbox{violet!11}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 05.  us modest recovery fed cut back qe next month reuters poll } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 06.  j.c. penney share spike report sale improve august } \\
    \colorbox{violet!9}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 07.  wallstreet end down fed uncertainty data boost europe } \\
    \colorbox{violet!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!17}{\makebox[3em]{\strut {0.18}}}  & \colorbox{green!79}{\makebox[3em]{\strut {0.79}}}  &  \colorbox{green!79}{\strut 08.  analysis balloon google experiment web access } \\
    \colorbox{violet!8}{\makebox[3em]{\strut {0.09}}}  & \colorbox{orange!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 09.  wallstreet fall uncertainty fed bond buying } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!16}{\makebox[3em]{\strut {0.16}}}  & \colorbox{green!5}{\makebox[3em]{\strut {0.05}}}  &  \colorbox{green!0}{\strut 10.  apple face possible may trial e book damage } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 11.  japan government spokesman no pm abe corporate tax cut } \\
    \midrule
          &       &       & Date: 2013-08-29 \\
    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 01.  india pm likely make statement economy friday } \\
    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 02.  boj warns emerge market may see outflow } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 03.  european rehn say lender step up assessment greece next month } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!20}{\makebox[3em]{\strut {0.20}}}  &  \colorbox{green!20}{\strut 04.  china environment min suspends approval cnpc } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!7}{\makebox[3em]{\strut {0.08}}}  &  \colorbox{green!0}{\strut 05.  italy still meet target scrap property tax say rehn } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!1}{\strut 06.  spain economic slump longer than thought but ease } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 07.  india central bank consider gold trade minister } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  rupee fall front slow indian economy } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 09.  india rupee bounce record low pm may address economy } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 10.  exclusive india might buy gold ease rupee crisis } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 11.  spain recession longer than thought but close end } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 12.  india finance minister asks bank ensure credit flow industry } \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 13.  easing stimulus weigh oil next year reuters poll } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 14.  exclusive india might buy gold ease rupee crisis } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 15.  india rupee bounce record low government seek solution } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!37}{\makebox[3em]{\strut {0.37}}}  &  \colorbox{green!37}{\strut 16.  china google power global drive } \\
    \colorbox{violet!09}{\makebox[3em]{\strut {0.09}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 17.  gdp growth beat forecast may boost case fed move } \\
    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.01}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 18.  wallstreet rise economy but syria concern limit gain } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.01}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 19.  oil dip syria action uncertain dollar rise data } \\
    \colorbox{violet!1}{\makebox[3em]{\strut {0.02}}}  & \colorbox{orange!0}{\makebox[3em]{\strut {0.00}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 20.  boe carney say uncertainty rbs future end } \\
    \bottomrule
    \end{tabular}%
  }
  \label{tab:GOOG-attn-Apnx}%
}
\end{table}



%\begin{table}[htbp]
%  \centering
%  \caption{AAPL dataset: News headlines from 3 days in 2013 (test set). Succinct set of relevant news in AsyncLSTM is blue-highlighted by setting: accumulated probability mass $\geq 50\%$.}
%  \resizebox{0.45\textwidth}{!}{%
%    \begin{tabular}{llll}
%    \toprule
%    GRUtxt & LSTMw/o & AsyncLSTM & News headlines \\
%    \midrule
%          &       &       & 1/22/13 \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!0}{\makebox[3em]{\strut {0.00}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  analysis no respite euro zone long rebalancing slog } \\
%    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!15}{\makebox[3em]{\strut {0.15}}}  &  \colorbox{green!0}{\strut 02.  japan government welcome boj ease step towards percent inflation } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 03.  japan government panel need achieve budget surplus } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!21}{\makebox[3em]{\strut {0.21}}}  &  \colorbox{green!21}{\strut 04.  instant view existing home sale fall december } \\
%    \colorbox{violet!14}{\makebox[3em]{\strut {0.14}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!8}{\makebox[3em]{\strut {0.09}}}  &  \colorbox{green!0}{\strut 05.  german exporter fear devaluation round boj move } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 06.  bank japan yet revive economy } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 07.  home resale fall housing recovery still track } \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  instant view google put up well than expect quarterly number } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 09.  bank japan buy asset sp set new five year high } \\
%    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 10.  google fourth quarter result shine ad rate decline slows } \\
%    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 11.  banks commodity stock lift sp five year high } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 12.  google fourth quarter result shine ad rate decline slows } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!13}{\makebox[3em]{\strut {0.14}}}  & \colorbox{green!39}{\makebox[3em]{\strut {0.40}}}  &  \colorbox{green!39}{\strut 13.  steve jobs threaten patent suit no hire policy filing } \\
%    \midrule
%          &       &       & 8/14/13 \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  france exit recession beat second quarter gdp forecast } \\
%    \colorbox{violet!9}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!14}{\makebox[3em]{\strut {0.14}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 02.  euro zone performance suggests recovery sight european rehn } \\
%    \colorbox{violet!14}{\makebox[3em]{\strut {0.14}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  germany france haul euro zone recession } \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  yellen see likely next fed chair despite summers chatter reuters poll } \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 05.  us modest recovery fed cut back qe next month reuters poll } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 06.  j.c. penney share spike report sale improve august } \\
%    \colorbox{violet!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 07.  wallstreet end down fed uncertainty data boost europe } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  analysis balloon google experiment web access } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 09.  wallstreet fall uncertainty fed bond buying } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!75}{\makebox[3em]{\strut {0.76}}}  &  \colorbox{green!75}{\strut 10.  apple face possible may trial e book damage } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!17}{\makebox[3em]{\strut {0.17}}}  &  \colorbox{green!0}{\strut 11.  japan government spokesman no pm abe corporate tax cut } \\
%    \midrule
%          &       &       & 9/6/13 \\
%    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!20}{\makebox[3em]{\strut {0.21}}}  &  \colorbox{green!20}{\strut 01.  china unicom telecom sell late iphone shortly us launch } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 02.  spain industrial output fall month july } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  french consumer confidence trade point improve outlook } \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  uk industrial output flat july trade deficit widens sharply } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 05.  boj kuroda room policy response tax hike hurt economy minute } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!5}{\makebox[3em]{\strut {0.05}}}  &  \colorbox{green!0}{\strut 06.  wind down market street funding amid regulatory pressure } \\
%    \colorbox{violet!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 07.  china able cope fed policy taper central bank head } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  instant view us august nonfarm payroll rise } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 09.  analysis fed shift syria crisis trading strategy } \\
%    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 10.  factbox three thing learn us job report } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!9}{\makebox[3em]{\strut {0.09}}}  &  \colorbox{green!0}{\strut 11.  g20 say economy recover but no end crisis yet } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 12.  us regulator talk european energy price probe } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 13.  wallstreet flat job data syria worry spur caution } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 14.  job growth disappoints offer note fed } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 15.  bond yield dollar fall us job data } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!37}{\makebox[3em]{\strut {0.37}}}  &  \colorbox{green!37}{\strut 16.  apple hit us injunction e books antitrust case } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 17.  wallstreet week ahead markets could turn choppy fed syria risk mount } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 18.  china buy giant kazakh oilfield billion } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!1}{\strut 19.  italy wo n't block foreign takeover economy minister } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 20.  china august export beat forecast point stabilization } \\
%    \colorbox{violet!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!06}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 21.  wallstreet week ahead markets could turn choppy fed syria risk mount } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 22.  india inc policymakers shape up ship } \\
%    \colorbox{violet!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.04}}}  &  \colorbox{green!0}{\strut 23.  cost lack indonesia economy } \\
%    \colorbox{violet!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 24.  mexico proposes new tax regime pemex } \\
%    \bottomrule
%    \end{tabular}%
%  }
%  \label{tab:addlabel}%
%\end{table}%
%





%\begin{table}[htbp]
%  \centering
%  \caption{GOOG dataset: News headlines from 3 days in 2013 (test set). Succinct set of relevant news in AsyncLSTM is blue-highlighted by setting: accumulated probability mass $\geq 50\%$.}
%  \resizebox{0.45\textwidth}{!}{%
%    \begin{tabular}{llll}
%    \toprule
%    GRUtxt & LSTMw/o & AsyncLSTM & News headlines \\
%    \midrule
%          &       &       & 1/9/13 \\
%    \colorbox{violet!23}{\makebox[3em]{\strut {0.23}}}  & \colorbox{orange!34}{\makebox[3em]{\strut {0.34}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  short sellers circle stock confidence waver } \\
%    \colorbox{violet!26}{\makebox[3em]{\strut {0.26}}}  & \colorbox{orange!52}{\makebox[3em]{\strut {0.52}}}  & \colorbox{green!87}{\makebox[3em]{\strut {0.87}}}  &  \colorbox{green!87}{\strut 02.  google drop key patent claim microsoft } \\
%    \colorbox{violet!21}{\makebox[3em]{\strut {0.21}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  alcoa result lift share dollar up vs. yen } \\
%    \colorbox{violet!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  wallstreet rise alcoa report earnings } \\
%    \midrule
%          &       &       & 8/14/13 \\
%    \colorbox{violet!10}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  france exit recession beat second quarter gdp forecast } \\
%    \colorbox{violet!9}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 02.  euro zone performance suggests recovery sight european rehn } \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.07}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  germany france haul euro zone recession } \\
%    \colorbox{violet!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  yellen see likely next fed chair despite summers chatter reuters poll } \\
%    \colorbox{violet!11}{\makebox[3em]{\strut {0.12}}}  & \colorbox{orange!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 05.  us modest recovery fed cut back qe next month reuters poll } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 06.  j.c. penney share spike report sale improve august } \\
%    \colorbox{violet!9}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 07.  wallstreet end down fed uncertainty data boost europe } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!17}{\makebox[3em]{\strut {0.18}}}  & \colorbox{green!79}{\makebox[3em]{\strut {0.79}}}  &  \colorbox{green!79}{\strut 08.  analysis balloon google experiment web access } \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.09}}}  & \colorbox{orange!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 09.  wallstreet fall uncertainty fed bond buying } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!16}{\makebox[3em]{\strut {0.16}}}  & \colorbox{green!5}{\makebox[3em]{\strut {0.05}}}  &  \colorbox{green!0}{\strut 10.  apple face possible may trial e book damage } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 11.  japan government spokesman no pm abe corporate tax cut } \\
%    \midrule
%          &       &       & 8/29/13 \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 01.  india pm likely make statement economy friday } \\
%    \colorbox{violet!7}{\makebox[3em]{\strut {0.07}}}  & \colorbox{orange!11}{\makebox[3em]{\strut {0.11}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 02.  boj warns emerge market may see outflow } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 03.  european rehn say lender step up assessment greece next month } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!20}{\makebox[3em]{\strut {0.20}}}  &  \colorbox{green!20}{\strut 04.  china environment min suspends approval cnpc } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!7}{\makebox[3em]{\strut {0.08}}}  &  \colorbox{green!0}{\strut 05.  italy still meet target scrap property tax say rehn } \\
%    \colorbox{violet!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!1}{\strut 06.  spain economic slump longer than thought but ease } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 07.  india central bank consider gold trade minister } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 08.  rupee fall front slow indian economy } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 09.  india rupee bounce record low pm may address economy } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 10.  exclusive india might buy gold ease rupee crisis } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 11.  spain recession longer than thought but close end } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 12.  india finance minister asks bank ensure credit flow industry } \\
%    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 13.  easing stimulus weigh oil next year reuters poll } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 14.  exclusive india might buy gold ease rupee crisis } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 15.  india rupee bounce record low government seek solution } \\
%    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!37}{\makebox[3em]{\strut {0.37}}}  &  \colorbox{green!37}{\strut 16.  china google power global drive } \\
%    \colorbox{violet!09}{\makebox[3em]{\strut {0.09}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 17.  gdp growth beat forecast may boost case fed move } \\
%    \colorbox{violet!8}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.01}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 18.  wallstreet rise economy but syria concern limit gain } \\
%    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.01}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 19.  oil dip syria action uncertain dollar rise data } \\
%    \colorbox{violet!1}{\makebox[3em]{\strut {0.02}}}  & \colorbox{orange!0}{\makebox[3em]{\strut {0.00}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.01}}}  &  \colorbox{green!0}{\strut 20.  boe carney say uncertainty rbs future end } \\
%    \end{tabular}%
%  }
%  \label{tab:addlabel}%
%\end{table}%
%




==> Exp_qualitative.tex <==

\vspace*{-0.2cm}
\subsection{Quantitative evaluation on prediction accuracy}   \label{AAPLGOOG-Accu}
\vspace*{-0.2cm}
We construct two datasets with the input modality for the time series is respectively selected from AAPL and GOOG stock series, while the textual data modality is the whole corpus of Reuters news headlines. Note that, stock name of the time series is not given to train our model. We use prediction accuracy as means to evaluate the high level performance of all models.
Table~\ref{tab:comp_acc} reports that evaluation in forecasting next day stock price movement (up/down) for the companies, while Table~\ref{tab:comp_time} presents the results when we vary the daily latest time up to which the news headlines are used by the models. Observations from these results are briefly summarized as follows: (i) Varying the latest time of collected news made less impact on prediction accuracy of all models (as compared to those seen in the S\&P500 summarized in Appendix~\ref{SP}); (ii) MSIN shows competitive performance against other techniques in both datasets, and its prediction accuracies are between 3\% to 6\% higher than the random guess. Two reasons can justify for these observations. First, daily news for these specific companies (statistics are shown in Appendix~\ref{GTn}) is not always available while the prediction is evaluated for every sample. Second, as shortly seen below, the news contents often report companies' events rather than stock price performance of company (contrasted to the market index S\&P500). 




%    Again, the most simple metric for evaluation is through the classification accuracy. Table~\ref{tab:comp_acc} reports the accuracy rates of all models in predicting the companies' stock price movement one day ahead, while Table~\ref{tab:comp_time} presents such evaluation when we vary the daily latest time up to which the news headlines are collected (similar to those evaluated with the S\&P500 series above). We briefly summarize these experiment's results: (i) Varying the latest time of collected news made less impact on prediction accuracy (as compared to S\&P500 time series); (ii) MSIN shows competitive performance against other models in both datasets, and its classification accuracies are between 3\% to 6\% higher than the random guess. There are two essential reasons to justify for these observations. First, unlike global index S\&P500 series which are frequently reported in the Reuters news corpus, we do not have daily news for each of these specific companies (as presented in Table~\ref{tab:stat}'s 2nd and 3rd columns) while the forecasting accuracy is still being evaluated at the daily basic. Second, news articles often report companies' events rather than its stock price performance as usually seen in the S\&P500's experiments.



\vspace*{-0.3cm}
\begin{table}[htbp]
\captionsetup{font=scriptsize}
\centering
  \caption{Classification performance on AAPL and GOOG.}
   \resizebox{0.49\textwidth}{!}{%
   \begin{tabular}{lccccccc}
    \toprule
          & \multicolumn{3}{c}{AAPL Price Movement} &       & \multicolumn{3}{c}{GOOG Price Movement} \\
\cmidrule{2-4}\cmidrule{6-8}    Method  & Acc.  & Pre.  & Rec.  &       & Acc.  & Pre.  & Rec. \\
    \midrule
    LSTMw/o & 53.0    & 53.9/50.5 & 57.2/49.4 &       & 52.3  & 50.2/55.9 & 60.2/45.1 \\
    LSTMpar & 52.3  & 52.9/47.3 & 58.9/42.2 &       & 51.8  & 49.2/54.0 & 46.8/55.7 \\
    GRUts & 52.5  & 53.8/48.3 & 56.8/47.4 &       & 52.2  & 51.2/\textbf{54.9} & 47.4/\textbf{56.8} \\
    GRUtxt & 51.2  & 54.1/47.2 & 67.7/35.9 &       & 51.1  & 49.3/54.5 & 57.6/47.1 \\
    CNNtxt & 51.8  & 55.8/48.2 & 51.1/53.2 &       & 50.9  & 49.9/54.3 & 67.6/37.4 \\
    SVM   & 51.9  & 52.9/46.4 & \textbf{67.1}/34.2 &       & 51.6  & 49.2/53.1 & \textbf{60.2}/44.3 \\
    MSIN & \textbf{53.9}  & \textbf{56.1}/\textbf{53.2} & 59.3/\textbf{49.9} &       & \textbf{52.5}  & \textbf{55.2}/51.3 & 53.9/51.2 \\
    \bottomrule
    \end{tabular}%
  \label{tab:comp_acc}%
}
\end{table}

\vspace*{-0.3cm}
\begin{table}[htbp]
\captionsetup{font=scriptsize}
\centering
  \caption{Accuracy as varying time up to which news is collected. GRUts is excluded as this model takes only time series for its input data.}
   \resizebox{0.49\textwidth}{!}{%
    \begin{tabular}{rrrrrrrrrr}
    \toprule
          & \multicolumn{4}{c}{AAPL }     &       & \multicolumn{4}{c}{GOOG} \\
\cmidrule{2-5}\cmidrule{7-10}     Method  & 9:00  & 15:40 & 19:00 & 23:59 &       & 9:00  & 15:00 & 19:00 & 23:59 \\
    \midrule
    LSTMw/o & 53.3  & 53.2  & 54.2  & 53.8  &       & 52.5  & 53.5  & 54.2  & 54.3 \\
    LSTMpar & 52.4  & 52.4  & 53.9  & 53.7  &       & 52.2  & 52.9  & 53.5  & 53.4 \\
    GRUtxt & 51.8  & 52.3  & 52.8  & 52.9  &       & 51.9  & 52.5  & 52.8  & 53.0 \\
    CNNtxt & 52.0  & 52.1  & 53.3  & 53.2  &       & 51.6  & 51.8  & 52.7  & 53.1 \\
    SVM   & 52.1  & 52.5  & 52.6  & 52.8  &       & 51.7  & 52.1  & 52.9  & 52.9 \\
    MSIN & \textbf{54.3}  & \textbf{54.8}  & \textbf{56.1}  & \textbf{55.9}  &       & \textbf{53.0}  & \textbf{53.4}  & \textbf{55.6}  & \textbf{55.8} \\
    \bottomrule
    \end{tabular}%
  \label{tab:comp_time}
}
\end{table}


%\begin{table}[htbp]
%  \centering
%  \caption{Classification performance on AAPL and GOOG.}
%   \resizebox{0.45\textwidth}{!}{%
%   \begin{tabular}{lccccccc}
%    \toprule
%          & \multicolumn{3}{c}{AAPL Price Movement} &       & \multicolumn{3}{c}{GOOG Price Movement} \\
%\cmidrule{2-4}\cmidrule{6-8}          & Acc.  & Pre.  & Rec.  &       & Acc.  & Pre.  & Rec. \\
%    \midrule
%    LSTMw/o & 53.0    & 53.9/50.5 & 57.2/49.4 &       & 52.3  & 50.2/55.9 & 60.2/45.1 \\
%    LSTMpar & 52.3  & 52.9/47.3 & 58.9/42.2 &       & 51.8  & 49.2/54.0 & 46.8/55.7 \\
%    GRUts & 52.5  & 53.8/48.3 & 56.8/47.4 &       & 52.2  & 51.2/54.9 & 47.4/56.8 \\
%    GRUtxt & 51.2  & 54.1/47.2 & 67.7/35.9 &       & 51.1  & 49.3/54.5 & 57.6/47.1 \\
%    CNNtxt & 51.8  & 55.8/48.2 & 51.1/53.2 &       & 50.9  & 49.9/54.3 & 67.6/37.4 \\
%    SVM   & 51.9  & 52.9/46.4 & 67.1/34.2 &       & 51.6  & 49.2/53.1 & 60.2/44.3 \\
%    MSIN & 53.9  & 56.1/53.2 & 59.3/49.9 &       & 52.5  & 55.2/51.3 & 53.9/51.2 \\
%    \bottomrule
%    \end{tabular}%
%   }
%  \label{tab:comp_acc}%
%\end{table}%
%
%
%
%\begin{table}[htbp]
%  \centering
%  \caption{Classification performance on AAPL and GOOG as varying the latest time up to which news headlines are collected.}
%   \resizebox{0.45\textwidth}{!}{%
%    \begin{tabular}{rrrrrrrrrr}
%    \toprule
%          & \multicolumn{4}{c}{AAPL }     &       & \multicolumn{4}{c}{GOOG} \\
%\cmidrule{2-5}\cmidrule{7-10}          & 9:00  & 15:40 & 19:00 & 23:59 &       & 9:00  & 15:00 & 19:00 & 23:59 \\
%    \midrule
%    LSTMw/o & 53.3  & 53.2  & 54.2  & 53.8  &       & 52.5  & 53.5  & 54.2  & 54.3 \\
%    LSTMpar & 52.4  & 52.4  & 53.9  & 53.7  &       & 52.2  & 52.9  & 53.5  & 53.4 \\
%    GRUtxt & 51.8  & 52.3  & 52.8  & 52.9  &       & 51.9  & 52.5  & 52.8  & 53.0 \\
%    CNNtxt & 52.0  & 52.1  & 53.3  & 53.2  &       & 51.6  & 51.8  & 52.7  & 53.1 \\
%    SVM   & 52.1  & 52.5  & 52.6  & 52.8  &       & 51.7  & 52.1  & 52.9  & 52.9 \\
%    MSIN & 54.3  & 54.8  & 56.1  & 55.9  &       & 53.0  & 53.4  & 55.6  & 55.8 \\
%    \bottomrule
%    \end{tabular}%
%     }
%  \label{tab:comp_time}%
%\end{table}%


%% Table generated by Excel2LaTeX from sheet 'PreRecall'
%\begin{table}[htbp]
%  \centering
%  \caption{Add caption}
%    \begin{tabular}{rrrrrrrrrr}
%    \toprule
%          & \multicolumn{4}{c}{AAPL }     &       & \multicolumn{4}{c}{GOOG} \\
%\cmidrule{2-5}\cmidrule{7-10}          & 9:00  & 15:40 & 19:00 & 23:59 &       & 9:00  & 15:00 & 19:00 & 23:00 \\
%    \midrule
%    LSTMw/o & 53.3  & 53.2  & 54.2  & 53.8  &       & 52.5  & 53.5  & 54.2  & 54.3 \\
%    LSTMpar & 52.4  & 52.4  & 53.9  & 53.7  &       & 52.2  & 52.9  & 53.5  & 53.4 \\
%    GRUtxt & 51.8  & 52.3  & 52.8  & 52.9  &       & 51.9  & 52.5  & 52.8  & 53.0 \\
%    CNNtxt & 52.0  & 52.1  & 53.3  & 53.2  &       & 51.6  & 51.8  & 52.7  & 53.1 \\
%    SVM   & 52.1  & 52.5  & 52.6  & 52.8  &       & 51.7  & 52.1  & 52.9  & 52.9 \\
%    MSIN & 54.3  & 54.8  & 56.1  & 55.9  &       & 53.0  & 53.4  & 55.6  & 55.8 \\
%    \bottomrule
%    \end{tabular}%
%  \label{tab:addlabel}%
%\end{table}%

%As noted, evaluating the quality of relevant news in association with a time series is a non-trivial task and prediction accuracy is a high-level metric for this task. We hence provide more insights into the models' performance through the precision and recall computed w.r.t. the news categories annotated with the company name. Such ground truth annotation fortunately can be extracted from the raw news filenames in the Reuter corpus, but note that such information is never given to our models during training. Some basic statistics about these news categories are given in Table~\ref{tab:stat}. 

%
%\begin{table}[htbp]
%  \centering
%  \caption{Add caption}
%  \resizebox{0.45\textwidth}{!}{%
%    \begin{tabular}{crrrrrrrr}
%    \toprule
%    Dataset & \%GTn & \%GTd & Avg\#GTn/GTd & Max\#GTn & \#News & \#NewsOnGTd & \#GTn & \#GTd \\
%    \midrule
%    AAPL  & 8\%   & 45\%  & 15\%  & 9     & 2202  & 1124  & 176   & 100 \\
%    GOOG  & 3.5\% & 26\%  & 12\%  & 5     & 2202  & 656   & 78    & 58 \\
%    \bottomrule
%    \end{tabular}%
%  }
%  \label{tab:stat}%
%\end{table}%

%We next investigate in depth the capability of discovering top most relevant news in association with each input stock time series. We hence make use of precision and recall computed w.r.t. the number of news articles annotated with the company name as the ground truth. These measures are also evaluated on the days (samples) that contain at least one news article associated with the corresponding company for better justification. In Fig.~\ref{fig:AAPL_PR} and~\ref{fig:GOOG_PR}, we plot these two measures respectively for the Apple and Google as the number of selected news headlines to be outputted is varied from 1 to 5





%\begin{figure}[t]
%\captionsetup{font=small}
%%\vspace{-6ex}
%  \begin{center}\hspace{-0.5cm}
%    \mbox{
%      \subfigure [] {\scalebox{0.34}{\epsfig{file=AAPLpre.pdf}}}\hspace{0.1cm}
%      \subfigure [] {\scalebox{0.34}{\epsfig{file=AAPLrec.pdf}}}
%      }\vspace{-2ex}
%\caption{Precision and Recall computed w.r.t. the news headlines annotated with ``apple'' by Reuters. They are calculated in relative to the maximum top relevant headlines returned.} \label{fig:AAPL_PR} %\vspace{6ex}
%  \end{center} \vspace{-2ex}
%\end{figure}

%
%\begin{figure}[t]
%\captionsetup{font=small}
%\vspace{-2ex}
%  \begin{center}\hspace{-0.5cm}
%    \mbox{
%      \subfigure [] {\scalebox{0.32}{\epsfig{file=GOOGpre.pdf}}}\hspace{0.1cm}
%      \subfigure [] {\scalebox{0.32}{\epsfig{file=GOOGrec.pdf}}}\hspace{0.1cm}
%      \subfigure [] {\scalebox{0.32} {\epsfig{file=b_GOOGa.pdf}}}
%      }\vspace{-2ex}
%\caption{Precision and Recall computed w.r.t. the news headlines annotated with ``google'' by Reuters. They are calculated in relative to the maximum top relevant headlines returned.} \label{fig:GOOG_PR} %\vspace{6ex}
%  \end{center} \vspace{-2ex}
%\end{figure}

==> GOOG-ATTN-SMALL.tex <==

\begin{table}%[htbp]
 \centering
  \caption{GOOG: News headlines from 3 days in 2013 (test set). Succinct set of relevant news in MSIN is blue-highlighted by setting: accumulated probability mass $\geq 50\%$.(ref. to Appendix~\ref{AG-ATTN-ALL})}
  \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}[t]{llll}
    \toprule
    GRUtxt & LSTMw/o & MSIN & News headlines \\
    \midrule
          &       &       & Date: 2013-01-09 \\
    \colorbox{violet!23}{\makebox[3em]{\strut {0.23}}}  & \colorbox{orange!34}{\makebox[3em]{\strut {0.34}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  short sellers circle stock confidence waver } \\
    \colorbox{violet!26}{\makebox[3em]{\strut {0.26}}}  & \colorbox{orange!52}{\makebox[3em]{\strut {0.52}}}  & \colorbox{green!87}{\makebox[3em]{\strut {0.87}}}  &  \colorbox{green!87}{\strut 02.  google drop key patent claim microsoft } \\
    \colorbox{violet!21}{\makebox[3em]{\strut {0.21}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 03.  alcoa result lift share dollar up vs. yen } \\
    \colorbox{violet!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 04.  wallstreet rise alcoa report earnings } \\
    \midrule
          &       &       & Date: 2013-08-14 \\
    \colorbox{violet!10}{\makebox[3em]{\strut {0.11}}}  & \colorbox{orange!10}{\makebox[3em]{\strut {0.10}}}  & \colorbox{green!0}{\makebox[3em]{\strut {0.00}}}  &  \colorbox{green!0}{\strut 01.  france exit recession beat second quarter gdp forecast } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{green!1}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 06.  j.c. penney share spike report sale improve august } \\
    \colorbox{violet!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{orange!17}{\makebox[3em]{\strut {0.18}}}  & \colorbox{green!79}{\makebox[3em]{\strut {0.79}}}  &  \colorbox{green!79}{\strut 08.  analysis balloon google experiment web access } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!16}{\makebox[3em]{\strut {0.16}}}  & \colorbox{green!5}{\makebox[3em]{\strut {0.05}}}  &  \colorbox{green!0}{\strut 10.  apple face possible may trial e book damage } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.04}}}  & \colorbox{orange!7}{\makebox[3em]{\strut {0.08}}}  & \colorbox{green!2}{\makebox[3em]{\strut {0.02}}}  &  \colorbox{green!0}{\strut 11.  japan government spokesman no pm abe corporate tax cut } \\
    \midrule
          &       &       & Date: 2013-08-29 \\
    \colorbox{violet!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!9}{\makebox[3em]{\strut {0.09}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 03.  european rehn say lender step up assessment greece next month } \\
    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!6}{\makebox[3em]{\strut {0.06}}}  & \colorbox{green!20}{\makebox[3em]{\strut {0.20}}}  &  \colorbox{green!20}{\strut 04.  china environment min suspends approval cnpc } \\
    \colorbox{violet!4}{\makebox[3em]{\strut {0.05}}}  & \colorbox{orange!12}{\makebox[3em]{\strut {0.12}}}  & \colorbox{green!7}{\makebox[3em]{\strut {0.08}}}  &  \colorbox{green!0}{\strut 05.  italy still meet target scrap property tax say rehn } \\    \colorbox{violet!3}{\makebox[3em]{\strut {0.03}}}  & \colorbox{orange!2}{\makebox[3em]{\strut {0.02}}}  & \colorbox{green!37}{\makebox[3em]{\strut {0.37}}}  &  \colorbox{green!37}{\strut 16.  china google power global drive } \\
    \colorbox{violet!5}{\makebox[3em]{\strut {0.06}}}  & \colorbox{orange!1}{\makebox[3em]{\strut {0.01}}}  & \colorbox{green!3}{\makebox[3em]{\strut {0.03}}}  &  \colorbox{green!0}{\strut 19.  oil dip syria action uncertain dollar rise data } \\
    \bottomrule
    \end{tabular}%
  }
  \label{tab:GOOG-attn}%
\end{table}

==> SP5-news.tex <==

%
%\begin{figure}[htbp]
%  \begin{minipage}[b]{0.5\linewidth}
%    \centering
%   \includegraphics[width=5cm]{NumhlinesPerDay.pdf}
%   \caption{Distribution of numbers of news headlines released per day by Thomson Reuters.}
%    \label{fig:chapter001_dist_001}
%     \begin{minipage}[b]{0.9\linewidth}
%    \centering
%    \caption{GOOG dataset:of news headlines released per day by Thomson Reuters}
%    \begin{tabular}[t]{ccc}
%    x & x & x\\
%    x & x & x
%  \end{tabular}
%  \label{tab:GOOG-attn2}%
%  \end{minipage}
%  \end{minipage}
%  \hspace{0.5cm}
%  \begin{minipage}[b]{0.5\linewidth}
%    \centering
%    \caption{GOOG dataset:}
%    \begin{tabular}[t]{ccc}
%    x & x & x\\
%    x & x & x
%  \end{tabular}
%  \label{tab:GOOG-attn2}%
%  \end{minipage}
%\end{figure}



\begin{table}%[htbp]
\captionsetup{font=scriptsize}
\parbox[t]{.37\linewidth}{
 \centering
% \vspace*{-0.7cm}
  \caption{Classification performance of all models on market movement (up/down) of S\&P500. Precision and recall are reported w.r.t. each of 2 class labels.}
  \vspace*{0.2cm}
    \resizebox{0.35\textwidth}{!}{%
   \begin{tabular}{cccc}
    \toprule
    Methods & Acc.  & Pre.  & Rec. \\
    \midrule
    LSTMw/o & 55.8  & \textbf{63.9}/48.2 & 56.1/\textbf{56.4} \\
    LSTMpar & 53.6  & 57.8/43.5 & 70.1/31.3 \\
    GRUts & 52.8  & 58.1/43.4 & 65.7/33.6 \\
    GRUtxt & 55.3  & 60.1/45.1 & 70.9/33.3 \\
    CNNtxt & 55.9  & 61.4/46.9 & 64.1/45.3 \\
    SVM   & 53.1  & 58.1/41.2 & \textbf{71.7}/27.4 \\
    AsyncLSTM & \textbf{56.4}  & 63.3/\textbf{50.1} & 56.9/56.3 \\
    \bottomrule
    \end{tabular}%
   }
  \label{tab:sp500Accuracy}%
  \centering
  \caption{Classification accuracy on S\&P500 as varying the latest time up to which news headlines are collected.}
  \vspace*{0.2cm}
   \resizebox{0.35\textwidth}{!}{%
    \begin{tabular}{crrrr}
    \toprule
    Methods & 9:00  & 15:40 & 19:00 & 23:59 \\
    \midrule
    LSTMw/o & 56.1  & 57.2  & 67.7  & 77.6 \\
    LSTMpar & 54.5  & 56.1  & 65.9  & 76.1 \\
    GRUtxt & 56.9  & 58.1  & 68.3  & 78.2 \\
    CNNtxt & 56.8  & \textbf{60.1}  & 69.1  & 78.4 \\
    SVM   & 54.3  & 55.8  & 61.2  & 75.9 \\
    AsyncLSTM & \textbf{57.1}  & 59.8  & \textbf{69.6}  & \textbf{79.3} \\
    \bottomrule
    \end{tabular}%
   }
  \label{tab:sp500TimeVarying}%
%  \centering
%  %\vspace*{-0.7cm}
%  \centering
%  \caption{Statistics on  ``groundtruth" news headlines (on test dataset). \%GTn shows \% ground truth news over all news. \%GTn shows \% days having at least one GTn. GTn/GTd shows average \% of GTn on GTd.}
%  \vspace*{0.1cm}
%   \resizebox{0.4\textwidth}{!}{%
%    \begin{tabular}{crrrr}
%    \toprule
%    Dataset & \%GTn & \%GTd & GTn/GTd & Max\#GTn \\
%    \midrule
%    AAPL  & 8\%   & 45\%  & 15\%  & 9 \\
%    GOOG  & 3.5\% & 26\%  & 12\%  & 5 \\
%    \bottomrule
%    \end{tabular}%
%   }
%  \label{tab:stat}%
}
\hfill
\parbox[t]{.6\linewidth}{
\centering
 \caption{News headlines from three days selected from the test set, along with the attention mass (annotated in the numeric columns) by: GRUtxt, LSTMw/o and AsyncLSTM. Colored headlines are relevant news outputted by our model based on setting the accumulated probability mass $\geq 50\%$.}
  \vspace*{0.1cm}
  \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{cccl}
    \toprule
    GRUtxt & LSTMw/o & AsyncLSTM & News headlines \\
    \midrule
%    -/-   & -/+   & -/-   &  Date: 2013-02-03 \\
       &    &    &  Date: 2013-02-03 \\
     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!53}{\makebox[3em]{\strut{0.53}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 01. china service slow uptick highlight recovery \\
     \colorbox{violet!8}{\makebox[3em]{\strut{0.08}}} &  \colorbox{orange!10}{\makebox[3em]{\strut{0.10}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 02. japan finance minister weak yen result not goal anti deflation policy \\
     \colorbox{violet!2}{\makebox[3em]{\strut{0.02}}} &  \colorbox{orange!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{green!18}{\makebox[3em]{\strut{0.18}}} & 03. france track meet percent growth target minister \\
     \colorbox{violet!5}{\makebox[3em]{\strut{0.05}}} &  \colorbox{orange!16}{\makebox[3em]{\strut{0.16}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 04. watch central banker say not \\
     \colorbox{violet!12}{\makebox[3em]{\strut{0.12}}} &  \colorbox{orange!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{green!8}{\makebox[3em]{\strut{0.08}}} & 05. us small business borrowing rise december but barely \\
     \colorbox{violet!28}{\makebox[3em]{\strut{0.28}}} &  \colorbox{orange!8}{\makebox[3em]{\strut{0.08}}} &  \colorbox{green!7}{\makebox[3em]{\strut{0.07}}} & 06. gauge us business investment plan edge low \\
     \colorbox{violet!15}{\makebox[3em]{\strut{0.15}}} &  \colorbox{orange!7}{\makebox[3em]{\strut{0.07}}} &  \colorbox{green!39}{\makebox[3em]{\strut{0.39}}} & \colorbox{green!39}{\strut 07. global share euro fall sharply renew euro zone fear} \\
     \colorbox{violet!30}{\makebox[3em]{\strut{0.30}}} &  \colorbox{orange!3}{\makebox[3em]{\strut{0.03}}} &  \colorbox{green!21}{\makebox[3em]{\strut{0.21}}} & \colorbox{green!21}{\strut 08. sp post bad day since november hill share sink} \\
\midrule
%    -/-   & -/-   & -/-   &   Date: 2013-04-26 \\
       &    &    &   Date: 2013-04-26 \\
     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 01. japan growth strategy fiscal plan g8 \\
     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 02. boj credibility test division emerge over inflation target \\
     \colorbox{violet!28}{\makebox[3em]{\strut{0.28}}} &  \colorbox{orange!4}{\makebox[3em]{\strut{0.04}}} &  \colorbox{green!1}{\makebox[3em]{\strut{0.01}}} & 03. consumer sentiment wane april \\
     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{green!5}{\makebox[3em]{\strut{0.05}}} & 04. economic growth gauge year high last week ecri \\
     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 05. microsoft get upper hand first google patent trial \\
     \colorbox{violet!2}{\makebox[3em]{\strut{0.02}}} &  \colorbox{orange!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{green!1}{\makebox[3em]{\strut{0.01}}} & 06. growth fall short forecast weakness ahead \\
     \colorbox{violet!22}{\makebox[3em]{\strut{0.22}}} &  \colorbox{orange!9}{\makebox[3em]{\strut{0.09}}} &  \colorbox{green!14}{\makebox[3em]{\strut{0.14}}} & 07. dollar fall yen bond yield decline \\
     \colorbox{violet!28}{\makebox[3em]{\strut{0.28}}} &  \colorbox{orange!80}{\makebox[3em]{\strut{0.80}}} &  \colorbox{green!73}{\makebox[3em]{\strut{0.73}}} & \colorbox{green!73}{\strut 08. wallstreet dip gdp but finish week high} \\
     \colorbox{violet!19}{\makebox[3em]{\strut{0.19}}} &  \colorbox{orange!4}{\makebox[3em]{\strut{0.04}}} &  \colorbox{green!5}{\makebox[3em]{\strut{0.05}}} & 09. wallstreet week ahead central bank data steer investor \\
    \midrule
%    +/+   & +/+   & +/+   &  Date:  2013-10-18 \\
       &    &    &  Date:  2013-10-18 \\
     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!2}{\makebox[3em]{\strut{0.02}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 01. china economy show sign slow september stats bureau \\
     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 02. china share up comfort data but still weekly loss \\
     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!8}{\makebox[3em]{\strut{0.08}}} &  \colorbox{green!1}{\makebox[3em]{\strut{0.01}}} & 03. china third quarter gdp growth fast year but outlook dim \\
     \colorbox{violet!2}{\makebox[3em]{\strut{0.02}}} &  \colorbox{orange!26}{\makebox[3em]{\strut{0.26}}} &  \colorbox{green!7}{\makebox[3em]{\strut{0.07}}} & 04. google third quarter beat ad volume grows stock flirt level \\
     \colorbox{violet!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{orange!11}{\makebox[3em]{\strut{0.11}}} &  \colorbox{green!3}{\makebox[3em]{\strut{0.03}}} & 05. schlumberger baker top estimate global drilling \\
     \colorbox{violet!26}{\makebox[3em]{\strut{0.26}}} &  \colorbox{orange!2}{\makebox[3em]{\strut{0.02}}} &  \colorbox{green!1}{\makebox[3em]{\strut{0.01}}} & 06. us data boon computer driven trading \\
     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 07. fed release delayed report industrial output october \\
     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 08. data delay add us inflation bond sale \\
     \colorbox{violet!20}{\makebox[3em]{\strut{0.20}}} &  \colorbox{orange!10}{\makebox[3em]{\strut{0.10}}} &  \colorbox{green!7}{\makebox[3em]{\strut{0.07}}} & 09. stock split wane may follow google 1,000 \\
     \colorbox{violet!6}{\makebox[3em]{\strut{0.06}}} &  \colorbox{orange!3}{\makebox[3em]{\strut{0.03}}} &  \colorbox{green!41}{\makebox[3em]{\strut{0.41}}} & \colorbox{green!41}{\strut 10. global stock gain dollar fall fed see stay course} \\
     \colorbox{violet!44}{\makebox[3em]{\strut{0.44}}} &  \colorbox{orange!31}{\makebox[3em]{\strut{0.31}}} &  \colorbox{green!39}{\makebox[3em]{\strut{0.39}}} & \colorbox{green!39}{\strut 11. sp break record google stock top earnings} \\
     \colorbox{violet!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{orange!3}{\makebox[3em]{\strut{0.03}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 12. google share break mobile pay \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:sp500visual}%
}
\end{table}




%\begin{table}[htbp]
%  \centering
%  \caption{\small{News headlines from three days selected from the test set, along with the attention mass (annotated in the numeric columns) by: GRUtxt, LSTMw/o and AsyncLSTM. Colored headlines are relevant news outputted by our model based on setting the accumulated probability mass $\geq 50\%$.}}
%  \vspace*{0.1cm}
%  \resizebox{0.5\textwidth}{!}{%
%    \begin{tabular}{cccl}
%    \toprule
%    GRUtxt & LSTMw/o & AsyncLSTM & News headlines \\
%    \midrule
%%    -/-   & -/+   & -/-   &  Date: 2013-02-03 \\
%       &    &    &  Date: 2013-02-03 \\
%     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!53}{\makebox[3em]{\strut{0.53}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 01. china service slow uptick highlight recovery \\
%     \colorbox{violet!8}{\makebox[3em]{\strut{0.08}}} &  \colorbox{orange!10}{\makebox[3em]{\strut{0.10}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 02. japan finance minister weak yen result not goal anti deflation policy \\
%     \colorbox{violet!2}{\makebox[3em]{\strut{0.02}}} &  \colorbox{orange!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{green!18}{\makebox[3em]{\strut{0.18}}} & 03. france track meet percent growth target minister \\
%     \colorbox{violet!5}{\makebox[3em]{\strut{0.05}}} &  \colorbox{orange!16}{\makebox[3em]{\strut{0.16}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 04. watch central banker say not \\
%     \colorbox{violet!12}{\makebox[3em]{\strut{0.12}}} &  \colorbox{orange!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{green!8}{\makebox[3em]{\strut{0.08}}} & 05. us small business borrowing rise december but barely \\
%     \colorbox{violet!28}{\makebox[3em]{\strut{0.28}}} &  \colorbox{orange!8}{\makebox[3em]{\strut{0.08}}} &  \colorbox{green!7}{\makebox[3em]{\strut{0.07}}} & 06. gauge us business investment plan edge low \\
%     \colorbox{violet!15}{\makebox[3em]{\strut{0.15}}} &  \colorbox{orange!7}{\makebox[3em]{\strut{0.07}}} &  \colorbox{green!39}{\makebox[3em]{\strut{0.39}}} & \colorbox{green!39}{\strut 07. global share euro fall sharply renew euro zone fear} \\
%     \colorbox{violet!30}{\makebox[3em]{\strut{0.30}}} &  \colorbox{orange!3}{\makebox[3em]{\strut{0.03}}} &  \colorbox{green!21}{\makebox[3em]{\strut{0.21}}} & \colorbox{green!21}{\strut 08. sp post bad day since november hill share sink} \\
%\midrule
%%    -/-   & -/-   & -/-   &   Date: 2013-04-26 \\
%       &    &    &   Date: 2013-04-26 \\
%     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 01. japan growth strategy fiscal plan g8 \\
%     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 02. boj credibility test division emerge over inflation target \\
%     \colorbox{violet!28}{\makebox[3em]{\strut{0.28}}} &  \colorbox{orange!4}{\makebox[3em]{\strut{0.04}}} &  \colorbox{green!1}{\makebox[3em]{\strut{0.01}}} & 03. consumer sentiment wane april \\
%     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{green!5}{\makebox[3em]{\strut{0.05}}} & 04. economic growth gauge year high last week ecri \\
%     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 05. microsoft get upper hand first google patent trial \\
%     \colorbox{violet!2}{\makebox[3em]{\strut{0.02}}} &  \colorbox{orange!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{green!1}{\makebox[3em]{\strut{0.01}}} & 06. growth fall short forecast weakness ahead \\
%     \colorbox{violet!22}{\makebox[3em]{\strut{0.22}}} &  \colorbox{orange!9}{\makebox[3em]{\strut{0.09}}} &  \colorbox{green!14}{\makebox[3em]{\strut{0.14}}} & 07. dollar fall yen bond yield decline \\
%     \colorbox{violet!28}{\makebox[3em]{\strut{0.28}}} &  \colorbox{orange!80}{\makebox[3em]{\strut{0.80}}} &  \colorbox{green!73}{\makebox[3em]{\strut{0.73}}} & \colorbox{green!73}{\strut 08. wallstreet dip gdp but finish week high} \\
%     \colorbox{violet!19}{\makebox[3em]{\strut{0.19}}} &  \colorbox{orange!4}{\makebox[3em]{\strut{0.04}}} &  \colorbox{green!5}{\makebox[3em]{\strut{0.05}}} & 09. wallstreet week ahead central bank data steer investor \\
%    \midrule
%%    +/+   & +/+   & +/+   &  Date:  2013-10-18 \\
%       &    &    &  Date:  2013-10-18 \\
%     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!2}{\makebox[3em]{\strut{0.02}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 01. china economy show sign slow september stats bureau \\
%     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 02. china share up comfort data but still weekly loss \\
%     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!8}{\makebox[3em]{\strut{0.08}}} &  \colorbox{green!1}{\makebox[3em]{\strut{0.01}}} & 03. china third quarter gdp growth fast year but outlook dim \\
%     \colorbox{violet!2}{\makebox[3em]{\strut{0.02}}} &  \colorbox{orange!26}{\makebox[3em]{\strut{0.26}}} &  \colorbox{green!7}{\makebox[3em]{\strut{0.07}}} & 04. google third quarter beat ad volume grows stock flirt level \\
%     \colorbox{violet!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{orange!11}{\makebox[3em]{\strut{0.11}}} &  \colorbox{green!3}{\makebox[3em]{\strut{0.03}}} & 05. schlumberger baker top estimate global drilling \\
%     \colorbox{violet!26}{\makebox[3em]{\strut{0.26}}} &  \colorbox{orange!2}{\makebox[3em]{\strut{0.02}}} &  \colorbox{green!1}{\makebox[3em]{\strut{0.01}}} & 06. us data boon computer driven trading \\
%     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 07. fed release delayed report industrial output october \\
%     \colorbox{violet!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{orange!0}{\makebox[3em]{\strut{0.00}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 08. data delay add us inflation bond sale \\
%     \colorbox{violet!20}{\makebox[3em]{\strut{0.20}}} &  \colorbox{orange!10}{\makebox[3em]{\strut{0.10}}} &  \colorbox{green!7}{\makebox[3em]{\strut{0.07}}} & 09. stock split wane may follow google 1,000 \\
%     \colorbox{violet!6}{\makebox[3em]{\strut{0.06}}} &  \colorbox{orange!3}{\makebox[3em]{\strut{0.03}}} &  \colorbox{green!41}{\makebox[3em]{\strut{0.41}}} & \colorbox{green!41}{\strut 10. global stock gain dollar fall fed see stay course} \\
%     \colorbox{violet!44}{\makebox[3em]{\strut{0.44}}} &  \colorbox{orange!31}{\makebox[3em]{\strut{0.31}}} &  \colorbox{green!39}{\makebox[3em]{\strut{0.39}}} & \colorbox{green!39}{\strut 11. sp break record google stock top earnings} \\
%     \colorbox{violet!1}{\makebox[3em]{\strut{0.01}}} &  \colorbox{orange!3}{\makebox[3em]{\strut{0.03}}} &  \colorbox{green!0}{\makebox[3em]{\strut{0.00}}} & 12. google share break mobile pay \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{tab:sp500visual}%
%\end{table} 



